One Vector is Not Enough: Entity-Augmented Distributional Semantics for Discourse Relations

Discourse relations bind smaller linguistic units into coherent texts. However, automatically identifying discourse relations is difficult, because it requires understanding the semantics of the linked arguments. A more subtle challenge is that it is not enough to represent the meaning of each argument of a discourse relation, because the relation may depend on links between lower-level components, such as entity mentions. Our solution computes distributional meaning representations by composition up the syntactic parse tree. A key difference from previous work on compositional distributional semantics is that we also compute representations for entity mentions, using a novel downward compositional pass. Discourse relations are predicted from the distributional representations of the arguments, and also of their coreferent entity mentions. The resulting system obtains substantial improvements over the previous state-of-the-art in predicting implicit discourse relations in the Penn Discourse Treebank.

==> coref.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\section{Discourse Relations and Coreference}

\begin{itemize}
\item In analyzing a discourse, it is frequently the case that we would recognize it as coherent, in that it would satisfy the formal definition of some coherence relation, if only we could assume certain noun phrases to be coreferential. \cite{hobbs1979coherence}
\item object coreference and event coreference \cite{danlos2001event,danlos2004event}. In this paper, we only focus on object coreference (?)
\item Use discourse structure to help identifying coreference \cite{hobbs1979coherence,cristea1999discourse}
\item Anything from here \cite{gordon1998representation}
\item Anything from here \cite{grosz1995centering}
\end{itemize}

Before presenting the semantic composition model, we would like to provide a few more discussion on the relationship between discourse relations and coreference. 

==> exp2.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\section{Evaluation on the first-level discourse relation}
We also evaluate the \modelname~on the first level discourse relations in the PDTB. 

\subsection{Experimental setup}

% -----------------------------------------
\paragraph{Data preparation} In this experiment, we target on the first-level PDTB discourse relations: \rela{Comparison}, \rela{Contingency}, \rela{Expansion} and \rela{Temporal}. In order to compare with exsiting work, we used section 2 - 20 of the PDTB as training set, and section 21 - 22 for testing, section 0 - 1 as development set to search over the parameter space. In addition, as suggested by \newcite{pitler2009automatic}, we included the instances of the \rela{EntRel} into the \rela{Expansion} relation as positive instances. 

% ------------------------------------------
\paragraph{Classification method}
We used the \modelname~with the downward composition procedure and the same surface features listed in section \ref{sec:implement}. Instead of employing a multi-class classifier for all four relations, we also used the One-vs-Rest scheme and trained four binary classifiers with the \modelname~model --- one for each first-level discourse relation. For each binary classifier, the development set were used to search over the parameter space defined in section \ref{sec:implement}, where F1 score was used as the criterion to select the optimal parameter setting. For training of each binary classifier,  we resampled training instances in each class inversely proportional to the number of instances in each class to handle the imbalance problem in the training set. The same strategy is also used in \cite{pitler2009automatic}.

\paragraph{Competitive systems}
We compare our model with several competitive systems on the first-level discourse relation identification. \newcite{pitler2009automatic} presented the first systemic model on the first-level implicit relation identification, with linguistically informed features, such as polarity tags, word pairs, etc. \newcite{park2012implicit} shows that the performance on one speicific relation could be improved by selecting an optimal feature set. For one particular discourse relation, F1 score is optimized by adding feature set until no improvement can be made. One the other hand, \cite{biran2013aggregated} shows that aggregating word pair features, which have the similar function on predicting relations, is better than using word pairs as features directly. Besides feature engineering, the way of discourse relation identification is to predict discourse connectives and then use the predicted connectives as additional features \cite{zhou2010predicting}. In experiments, we compare the performance of our model with all four competitive systems.

% ------------------------------------------
\subsection{Experimental results}

\input{tab-levelone}

Table \ref{tab:level-one} presents the performance of the \modelname~model and the competitive systems. As shown in this table, our model fully outperform all competitive systems. Especially, our model achieve 4.52\% (on \rela{Comparison}), 1.57\% (on \rela{Contingency}), 0.69\% (on \rela{Expansion}), 0.34\% (on \rela{Temporal}) F1 score improvement over the state-of-the-art system from~\cite{park2012implicit} without selecting features for each discourse relation (and also each binary classifier) respectively. On accuracy, our model also gives the best results on three relations: \rela{Contingency}, \rela{Expansion} and \rela{Temporal}, while the best results on \rela{Comparison} is from \cite{park2012implicit}. 

As we already show that the prediction power of our model on the second level discourse relation identification, the results in Table \ref{tab:level-one} provide further evidence that our model could be used a implicit discourse relation identification system across two different levels. 

\yfcomment{I am not sure how to explain the result on \rela{Expansion}, as we include all the instances with \rela{EntRel} as positive examples. It looks like we should get better results on this relation identification. I will take a look into the data and the confusion matrix to see whether I can find an explanation.}

==> figures/fig-order.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\begin{figure*}
\centering
\begin{tikzpicture}[->,node distance=12pt,semithick]
\matrix [column sep=1em]{
  \node[draw,fill={rgb:yellow,1}](u1){$\uvec{1}$};
&  \node[draw,fill={rgb:yellow,1}](u2){$\uvec{2}$};
&  \node[draw,fill={rgb:yellow,1}](u3){$\uvec{3}$};
&  \node[draw,fill={rgb:yellow,1}](u4){$\uvec{4}$};
&  \node[draw,fill={rgb:yellow,1}](u5){$\uvec{5}$};
&  \node[draw,fill={rgb:yellow,1}](u6){$\uvec{6}$};
&  \node[draw,fill={rgb:yellow,1}](u7){$\uvec{7}$};
&  \node[draw,fill={rgb:yellow,1}](u8){$\uvec{8}$};
&  \node[draw,fill={rgb:red,1;blue,1}](u9){$\uvec{9}=\dvec{9}$};
&  \node[draw,fill={rgb:red,1}](d8){$\dvec{8}$}; 
&  \node[draw,fill={rgb:red,1}](d7){$\dvec{7}$}; 
&  \node[draw,fill={rgb:red,1}](d3){$\dvec{3}$}; 
\\
};
\path 
(u1) edge [bend left] (u9)
(u8) edge [bend left] (u9)
(u2) edge [bend left] (u8)
(u7) edge [bend left] (u8)
(u3) edge [bend left] (u7)
(u6) edge [bend left] (u7)
(u4) edge [bend left] (u6)
(u5) edge [bend left] (u6)
(u9) edge [bend right] (d8)
(u1) edge [bend right] (d8)
(d8) edge [bend right] (d7)
(u2) edge [bend right] (d7)
(u6) edge [bend right] (d3)
(d7) edge [bend right] (d3)
;
\end{tikzpicture}
\caption{A total ordering on the upward and downward nodes in Figure~\ref{fig:updown}, with arrows indicating how the representation at each node is computed for the sentence (a) and entity \entity{Michael}. Color \textcolor{blue}{blue} indicates the nodes from upward composition procedure, color \textcolor{red}{red} indicates the nodes from downward composition procedure. All arrows follow the ordering, indicating that the graph is acyclic.}
\label{fig:ordering}
\end{figure*}


==> figures/fig-parse.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\begin{figure*}
\centering
\subfigure[Upward composition procedure]{
  % \begin{tikzpicture}[scale=0.62]
  %   \Tree [.Arg1 [.S($\uvec{9}$) [.NP($\uvec{1}$) The~heightened~competition ] [.VP($\uvec{8}$) [.MD($\uvec{2}$) will ] [.VP($\uvec{7}$) [.VB($\uvec{3}$) hit ] [.NP($\uvec{6}$) [.NP($\uvec{4}$) IBM ] [.PP($\uvec{5}$) at~a~difficult~time ] ] ] ] ] ] ] ] ]
  %   % \Tree [.S($\uvec{9}$) [.NP($\uvec{1}$) Susan ] [.VP($\uvec{8}$) [.VBD($\uvec{2}$) gave ] [.NP($\uvec{7}$) [.NP($\uvec{3}$) Michelle ] [.NP($\uvec{6}$) [.DT($\uvec{4}$) the ] [.NN($\uvec{5}$) bagel ] ] ] ] ]
  % \end{tikzpicture}
  \includegraphics[width=7.5cm]{figures/upward.pdf}
  \label{fig:up}
}
\hskip 0.0cm
\subfigure[Downward composition procedure]{
  % \begin{tikzpicture}[scale=0.62]
  %   \Tree [.IBM [.NP($\dvec{4}$) [.NP($\dvec{6}$) [.VP($\dvec{7}$) [.VP($\dvec{8}$) [.S($\dvec{9}$) ] [.NP($\uvec{1}$) The~heightened~competition ]  ] [.MD($\uvec{2}$) will ] ] [.VB($\uvec{3}$) hit ] ] [.PP($\uvec{5}$) at~a~difficult~time ] ] ]
  %   % \Tree [.Michelle [.NP($\dvec{3}$) [.NP($\dvec{7}$) [.VP($\dvec{8}$) [.S($\dvec{9}[=\uvec{9}]$) ] [.NP($\uvec{1}$) Susan ] ] [.VBD($\uvec{2}$) gave ] ] [.NP($\uvec{6}$) [.DT($\uvec{4}$) the ] [.NN($\uvec{5}$) bagel ] ] ] ]
  % \end{tikzpicture}
  \includegraphics[width=7.5cm]{figures/downward.pdf}
  \label{fig:down}
}
\caption{An example parse tree, with numbered nodes. We collapsed all unary production rules, such as \emph{NN $\rightarrow$ NNP}. For the root note in the downward composition procedure, we set $\dvec{9}=\uvec{9}$.}
\label{fig:updown}
\end{figure*}

==> tab-ontonotes.tex <==

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "main"
%%% End: 

\begin{table*}
  \centering
  {% \small
  \begin{tabular}{lllllll}
    \hline
    Model & +Downward & Training Data  & Coreference & $K$ & Accuracy(\%) \\
    \hline
    1. SFM & & \ontodata-Tr  & & & 35.59\\[0.2em]
    2. \modelname & Yes & PDTB-Tr &  Automatic & 50 & 39.85 \\[0.2em]
    3. \modelname & No & \ontodata-Tr  & Automatic & 20 & 36.34 \\
    4. \modelname & Yes & \ontodata-Tr  & Automatic & 20 & 36.84 \\[0.2em]
    5. \modelname & No & \ontodata-Tr  & Gold  & 20 & 37.09\\
    6. \modelname& Yes & \ontodata-Tr  & Gold  & 20 & 38.84 \\
    \hline
  \end{tabular}
  }
  \caption{Experimental results with different training data and coreference annotation systems. All results are reported on the \ontodata~test data with the same coreference annotation method used in the training data. The \modelname~are trained with the all surface features listed in text.}
  \label{tab:results-ontonotes}
\end{table*}
